Inferring Latent Class Statistics from Text for Robust Visual Few-Shot Learning

In the realm of few-shot learning, foundation models like CLIP have proven effective but exhibit limitations in cross-domain robustness especially in few-shot settings. Recent works add text as an extra modality to enhance the performance of these models. Most of these approaches treat text as an auxiliary modality without fully exploring its potential to elucidate the underlying class visual features distribution. In this paper, we present a novel approach that leverages text-derived statistics to predict the mean and covariance of the visual feature distribution for each class. This predictive framework enriches the latent space, yielding more robust and generalizable few-shot learning models. We demonstrate the efficacy of incorporating both mean and covariance statistics in improving few-shot classification performance across various datasets. Our method shows that we can use text to predict the mean and covariance of the distribution offering promising improvements in few-shot learning scenarios.

==> plots/figure.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp010876175640308405] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.11 ][fill={rgb, 255:red, 255; green, 242; blue, 51 }  ,fill opacity=0.37 ][line width=0.75]  (522,83.75) -- (668,83.75) -- (668,227.25) -- (522,227.25) -- cycle ;
%Shape: Rectangle [id:dp7212112974195928] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (15.88,158.41) -- (118.33,158.41) -- (118.33,203.33) -- (15.88,203.33) -- cycle ;
%Shape: Rectangle [id:dp11765677141865982] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (10.64,162.89) -- (113.09,162.89) -- (113.09,207.81) -- (10.64,207.81) -- cycle ;
%Shape: Rectangle [id:dp8893093411644564] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (6,167.01) -- (108.45,167.01) -- (108.45,211.93) -- (6,211.93) -- cycle ;
%Shape: Trapezoid [id:dp5826320378046181] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 182; blue, 252 }  ,fill opacity=1 ] (134.15,139.61) -- (186.8,155.84) -- (186.38,211.03) -- (133.48,226.46) -- cycle ;
%Shape: Rectangle [id:dp7045152057321613] 
\draw  [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=0.77 ][fill={rgb, 255:red, 220; green, 124; blue, 235 }  ,fill opacity=1 ] (205.22,137.02) -- (226.83,137.02) -- (226.83,181.94) -- (205.22,181.94) -- cycle ;
%Shape: Rectangle [id:dp5413494659966478] 
\draw  [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=0.77 ][fill={rgb, 255:red, 220; green, 124; blue, 235 }  ,fill opacity=1 ] (205.22,189.64) -- (226.83,189.64) -- (226.83,234.57) -- (205.22,234.57) -- cycle ;
%Straight Lines [id:da5168089948320354] 
\draw    (233.69,161.17) -- (255.72,161.17) ;
\draw [shift={(257.72,161.17)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da20262334789168635] 
\draw    (233.69,213.8) -- (255.72,213.8) ;
\draw [shift={(257.72,213.8)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3176967888993163] 
\draw [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ]   (216.53,104.23) -- (216.53,128.98) ;
\draw [shift={(216.53,130.98)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8224396218177947] 
\draw    (301.27,24) -- (304.06,278.5) ;
%Image [id:dp943220156196493] 
\draw (376.04,46.32) node  {\includegraphics[width=31.7pt,height=29.6pt]{figures/17.23.09.png}};
%Image [id:dp14535528037455459] 
\draw (333.77,46.32) node  {\includegraphics[width=31.7pt,height=29.6pt]{figures/17.22.50.png}};
%Image [id:dp860815294891212] 
\draw (476.87,46.32) node  {\includegraphics[width=31.7pt,height=29.6pt]{figures/17.20.43.png}};
%Image [id:dp8070496361463122] 
\draw (434.6,46.32) node  {\includegraphics[width=31.7pt,height=29.6pt]{figures/17.20.54.png}};
%Shape: Trapezoid [id:dp5718924567141752] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 126; green, 182; blue, 252 }  ,fill opacity=1 ] (463.92,74.18) -- (455.67,102.26) -- (356.79,102.83) -- (348.22,74.84) -- cycle ;
%Shape: Polygon [id:ds5147844306775471] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=0.11 ][fill={rgb, 255:red, 205; green, 255; blue, 211 }  ,fill opacity=1 ] (668.44,160.11) -- (668,236.5) -- (599,236.5) -- (522,236.5) -- (521.78,159.89) -- cycle ;
%Image [id:dp17441125448829253] 
\draw (561.9,201.84) node  {\includegraphics[width=28.9pt,height=28.53pt]{figures/17.21.07.png}};
%Image [id:dp027828923356282287] 
\draw (550.57,133.24) node  {\includegraphics[width=28.9pt,height=28.53pt]{figures/17.22.58.png}};
%Image [id:dp3405547611021731] 
\draw (640.06,116.35) node  {\includegraphics[width=28.9pt,height=28.53pt]{figures/17.43.35.png}};
%Shape: Right Angle [id:dp8365161639052971] 
\draw  [color={rgb, 255:red, 66; green, 228; blue, 83 }  ,draw opacity=1 ] (580,152.67) -- (530.98,152.26) -- (531.3,114.22) ;
%Shape: Circle [id:dp2411118479388299] 
\draw  [color={rgb, 255:red, 228; green, 66; blue, 66 }  ,draw opacity=1 ][fill={rgb, 255:red, 66; green, 228; blue, 83 }  ,fill opacity=1 ] (573,152.67) .. controls (573,150.73) and (574.57,149.17) .. (576.5,149.17) .. controls (578.43,149.17) and (580,150.73) .. (580,152.67) .. controls (580,154.6) and (578.43,156.17) .. (576.5,156.17) .. controls (574.57,156.17) and (573,154.6) .. (573,152.67) -- cycle ;
%Shape: Rectangle [id:dp15639178973108003] 
\draw  [color={rgb, 255:red, 255; green, 242; blue, 51 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 242; blue, 51 }  ,fill opacity=0 ] (312.64,26.59) -- (397.17,26.59) -- (397.17,66.06) -- (312.64,66.06) -- cycle ;
%Shape: Rectangle [id:dp41590198903294673] 
\draw  [color={rgb, 255:red, 205; green, 255; blue, 211 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 242; blue, 51 }  ,fill opacity=0 ] (413.47,26.59) -- (498,26.59) -- (498,66.06) -- (413.47,66.06) -- cycle ;
%Shape: Right Angle [id:dp8275475997749389] 
\draw  [color={rgb, 255:red, 255; green, 193; blue, 51 }  ,draw opacity=1 ] (614.91,135) -- (659.33,135.37) -- (659.65,97.71) ;
%Shape: Circle [id:dp127002837122679] 
\draw  [color={rgb, 255:red, 255; green, 193; blue, 51 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 193; blue, 51 }  ,fill opacity=1 ] (611.41,135) .. controls (611.41,133.07) and (612.98,131.5) .. (614.91,131.5) .. controls (616.85,131.5) and (618.41,133.07) .. (618.41,135) .. controls (618.41,136.93) and (616.85,138.5) .. (614.91,138.5) .. controls (612.98,138.5) and (611.41,136.93) .. (611.41,135) -- cycle ;
%Shape: Right Angle [id:dp1121507628933851] 
\draw  [color={rgb, 255:red, 66; green, 228; blue, 83 }  ,draw opacity=1 ] (591.22,220.73) -- (542.31,220.32) -- (542.63,182.83) ;
%Shape: Circle [id:dp18638603990552616] 
\draw  [color={rgb, 255:red, 66; green, 228; blue, 83 }  ,draw opacity=1 ][fill={rgb, 255:red, 66; green, 228; blue, 83 }  ,fill opacity=1 ] (584.22,220.73) .. controls (584.22,218.8) and (585.79,217.23) .. (587.72,217.23) .. controls (589.66,217.23) and (591.22,218.8) .. (591.22,220.73) .. controls (591.22,222.66) and (589.66,224.23) .. (587.72,224.23) .. controls (585.79,224.23) and (584.22,222.66) .. (584.22,220.73) -- cycle ;
%Shape: Right Angle [id:dp6890033234524873] 
\draw  [color={rgb, 255:red, 66; green, 228; blue, 83 }  ,draw opacity=1 ] (610.7,178.32) -- (659.26,177.96) -- (659.54,215.91) ;
%Shape: Circle [id:dp10950829535617945] 
\draw  [color={rgb, 255:red, 66; green, 228; blue, 83 }  ,draw opacity=1 ][fill={rgb, 255:red, 66; green, 228; blue, 83 }  ,fill opacity=1 ] (617.69,178.21) .. controls (617.73,180.14) and (616.18,181.74) .. (614.25,181.77) .. controls (612.32,181.8) and (610.73,180.25) .. (610.7,178.32) .. controls (610.67,176.39) and (612.21,174.8) .. (614.14,174.77) .. controls (616.07,174.74) and (617.66,176.28) .. (617.69,178.21) -- cycle ;
%Straight Lines [id:da5090665515286381] 
\draw [color={rgb, 255:red, 220; green, 124; blue, 235 }  ,draw opacity=1 ]   (522,112.43) -- (581.91,135.64) -- (668,169) ;
%Image [id:dp8980978484347972] 
\draw (639.99,196.98) node  {\includegraphics[width=28.9pt,height=28.53pt]{figures/17.43.51.png}};

% Text Node
\draw (10.57,172.91) node [anchor=north west][inner sep=0.1pt]   [align=left] {{\tiny Its short crest and the upper}\\{\tiny parts of its plumage are blue }\\{\tiny while its belly is whitish gray}};
% Text Node
\draw (137.22,166.67) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{33.5pt}\setlength\topsep{0pt}
\begin{center}
{\small Text }\\{\small Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (207.39,201.28) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{15.06pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle g_{\Sigma }$
\end{center}

\end{minipage}};
% Text Node
\draw (263.31,149.11) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{13.5pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle \hat{\mu }_{t}$
\end{center}

\end{minipage}};
% Text Node
\draw (261.52,199.73) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{14.35pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle \hat{\Sigma }_{t}$
\end{center}

\end{minipage}};
% Text Node
\draw (207.46,149.52) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{14.47pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle g_{\mu }$
\end{center}

\end{minipage}};
% Text Node
\draw (134.49,84.02) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 155; green, 155; blue, 155 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{101.89pt}\setlength\topsep{0pt}
\begin{center}
Trained on base classes
\end{center}

\end{minipage}};
% Text Node
\draw (398.25,35.71) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{11.23pt}\setlength\topsep{0pt}
\begin{center}
...
\end{center}

\end{minipage}};
% Text Node
\draw (359.82,80.28) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{61.05pt}\setlength\topsep{0pt}
\begin{center}
{\small Image \ Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (396.61,107.26) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{14.85pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle \hat{\mu }_{v}$
\end{center}

\end{minipage}};
% Text Node
\draw (345.53,148.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{76.79pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle ( 1-\alpha )\hat{\mu }_{v} +\alpha \hat{\mu }_{t}$
\end{center}

\end{minipage}};
% Text Node
\draw (356.72,199.54) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{68.4pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle ( 1-\beta ) I+\alpha \hat{\Sigma }_{t}$
\end{center}

\end{minipage}};
% Text Node
\draw (95.62,252.05) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{66.01pt}\setlength\topsep{0pt}
\begin{center}
\textit{Learning phase}
\end{center}

\end{minipage}};
% Text Node
\draw (361.49,248.59) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{74.18pt}\setlength\topsep{0pt}
\begin{center}
\textit{Adaptation phase}
\end{center}

\end{minipage}};
% Text Node
\draw (-10.62,224.33) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{100.64pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Class description}
\end{center}
\end{minipage}};


% Text Node
\draw (558.16,247.67) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\begin{minipage}[lt]{56.8pt}\setlength\topsep{0pt}
\begin{center}
Classification
\end{center}

\end{minipage}};


\end{tikzpicture}

==> tables/MSE.tex <==
\begin{table}[!htbp]
\label{table:MSE
}
\centering
 \captionsetup{justification=centering}
  \begin{minipage}{0.9\linewidth}
\caption{Mean Squared Error of predictions}
\begin{tabular}{lllllll}
\cmidrule(r){2-7}
 & \multicolumn{3}{c}{$\bm{\mu}$}        & \multicolumn{3}{c}{$\mathbf{\Sigma}$}     \\
\cmidrule(r){2-4} \cmidrule(r){5-7}
Model             & train         & test          & val           & train         & test          & val           \\
\midrule
Baseline          & 0.99          & 1             & 0.99          & 1             & 1             & 1             \\
Class labels      & 0.49          & 0.62          & 0.61          & 0.62          & 0.8           & 0.8           \\
Class description & \textbf{0.34} & \textbf{0.39} & \textbf{0.39} & \textbf{0.55} & \textbf{0.67} & \textbf{0.67}\\
\bottomrule
\end{tabular}
\end{minipage}
\end{table}

==> tables/MSE_indomain_crossdomain_confs.tex <==
\begin{table}[!htbp]
\centering
 %\captionsetup{justification=centering}
 \scalebox{0.9}{
  \begin{minipage}{1\linewidth}
\begin{center}
\begin{tabular}{cllllllll}
\cmidrule(r){4-9}
& & & \multicolumn{3}{c}{$\bm{\mu}$}        & \multicolumn{3}{c}{$\mathbf{\Sigma}$}     \\
\cmidrule(r){4-6} \cmidrule(r){7-9}
 & & Model             & train         & val          & test           & train         & val          & test           \\
\midrule
\multirow{6}{*}{\rotatebox{90}{ImageNet}} & \multirow{3}{*}{\rotatebox{90}{ID}} & Baseline          & $1.00\pm0.00$          & $1.00\pm0.02$   
 & $0.98\pm0.02$  & $1.00\pm0.00$ & $1.01\pm0.05$             & $1.00\pm0.04$ \\
& & Class labels      & $0.07\pm0.00$  & $0.44\pm0.02$  & $0.45\pm0.01$          & $0.08\pm0.00$  & $0.70\pm0.03$ & $0.74\pm0.04$  \\
& & Class description & $0.07\pm0.00$ & $0.46\pm0.02$ & $0.47\pm0.01$ & $0.09\pm0.00$ & $0.70\pm0.03$ & $0.74\pm0.04$\\
%\midrule
\cmidrule(r){2-9}

 & \multirow{3}{*}{\rotatebox{90}{CD}} & Baseline          & $1.00\pm0.00$ & $0.99\pm0.03$ &  $1.67\pm0.10$  &               $1.00\pm0.00$ & $1.04\pm0.07$ & $4.99\pm0.90$ \\
& & Class labels  & $0.06\pm0.00$ & $0.43\pm0.03$ & $1.26\pm0.11$   & $0.09\pm0.01$ & $0.72\pm0.06$   & $3.99\pm0.60$ \\
& & Class description & $0.07\pm0.00$ & $0.45\pm0.02$ & $1.30\pm0.11$ & $0.09\pm0.01$ & $0.70\pm0.05$ & $4.67\pm0.84$\\
\cmidrule(r){1-9}

\multirow{3}{*}{\rotatebox{90}{iNat}} & \multirow{3}{*}{\rotatebox{90}{ID}} & Baseline          & $1.00\pm 0$.00 & $1.00\pm0.02$ & $0.97\pm0.02$         & $1.00\pm 0$.00             & $1.00\pm0.03$             & $0.99\pm0.03$              \\

& & Class labels      & $0.18\pm0.00$          & $0.60\pm0.02$  & $0.98\pm0.03$ & $0.28\pm0.00$  & $0.66\pm0.03$ & $0.72\pm0.03$  \\

& & Class description & $0.14\pm0.00$ & $0.42\pm0.01$ & $0.42\pm0.01$ & $0.25\pm0.00$ & $0.54\pm0.02$ & $0.56\pm0.02$\\
\bottomrule
\end{tabular}
\end{center}
\end{minipage}
}
\vspace{2mm}
\caption{Mean Squared Error of predictions from ImageNet-1k and iNaturalist. The baseline is the average value over the training set. We experiment with both in-domain (ID) and cross-domain (CD) settings. \textcolor{red}{will add confidence intervals}}
\label{table:MSE_indomain_crossdomain}
\end{table}

==> tables/cross_modal_openclass.tex <==
\newcommand{\uparrowgreen}{\tikz{\draw[green,->] (0,0) -- ++(0,0.3);}}
\newcommand{\downarrowred}{\tikz{\draw[red,->] (0,0.3) -- ++(0,-0.3);}}
\begin{table}[htbp]
\centering
 %\captionsetup{justification=centering}
\scalebox{0.52}{\begin{tabular}{c|c|cccccccccc|c}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Shots} & \multicolumn{11}{c}{Dataset}  \\ 
\cmidrule(r){3-13}
& & Caltech & EuroSAT & Food & Flowers & SUN397 & DTD  & Aircraft & Pets & Cars & UCF101 & Average \\ 

\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Baseline}} 
& 1 & $89.74\pm0.47$ & $81.34\pm0.66$ & $83.34\pm0.66$ & $90.92\pm0.42$ & $89.18\pm0.55$ & $71.23\pm0.66$ &  & $81.47\pm0.56$ & $90.31\pm0.42$ & $84.70\pm0.51$ &  \\
& 2 & $93.31\pm0.30$ &  $85.79\pm0.47$& $87.59\pm0.38$ & $94.66\pm0.21$ & $94.37\pm0.33$ & $76.36\pm0.56$ &  & $86.16\pm0.33$ & $94.28\pm0.29$ & $88.63\pm0.42$ &  \\
& 4 & $94.95\pm0.19$ & $88.60\pm0.35$ & $89.54\pm0.27$ & $96.38\pm0.14$ & $96.47\pm0.18$ & $79.53\pm0.37$ &  & $88.11\pm0.20$ & $96.04\pm0.17$ & $90.70\pm0.24$ &  \\
& 8 & $95.89\pm0.12$ & $89.85\pm0.23$ & $90.36\pm0.20$ & $97.09\pm0.09$ & $97.51\pm0.10$ & $80.88\pm0.25$ &  & $88.83\pm0.17$ & $96.78\pm0.11$ & $91.72\pm0.17$ &  \\
& 16 & $96.49\pm0.06$ & $90.39\pm0.17$ &$90.79\pm0.14$  & $97.51\pm0.04$ & $97.83\pm0.05$ & $81.63\pm0.17$ &  & $89.21\pm0.11$ & $97.12\pm0.06$ & $92.25\pm0.11$ &  \\
\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Mean from text}} 
& 1 &  &  &  &  &  &  &  &  &  &  &  \\
& 2 &  & &  &  &  &  &  &  &  &  &  \\
& 4 &  &  &  &  &  &  &  &  &  &  &  \\
& 8 &  &  &  &  &  &  &  &  &  &  &  \\
& 16 &  &  &  &  &  &  &  &  &  &  &  \\

 \midrule
\multirow{5}{*}{\parbox{2cm}{\centering Covariance from text}} 

& 1 &  &  &  &  &  &  &  &  &  &  &  \\
& 2 &  &  &  &  &  &  &  &  &  &  &  \\
& 4 &  &  &  &  &  &  &  &  &  &  &  \\
& 8 &  &  &  &  &  &  &  &  &  &  &  \\
& 16 &  &  &  &  &  &  &  &  &  &  &  \\

\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Mean and covariance from text}} 
& 1 & $93.56\pm0.32$ & $82.81\pm0.60$ & $86.95\pm0.47$ & $94.91\pm0.27$ & $92.03\pm0.36$ & $71.40\pm0.63$ &  & $89.90\pm0.12$ & $92.64\pm0.29$ & $86.07\pm0.43$ &  \\
& 2 & $95.38\pm0.21$ & $87.24\pm0.43$ & $90.68\pm0.29$ & $97.20\pm0.14$ & $94.71\pm0.30$ & $76.36\pm0.56$ &  & $90.34\pm0.12$ & $95.94\pm0.20$ & $88.74\pm0.40$ &  \\
& 4 & $96.47\pm0.14$ & $89.87\pm0.31$ & $92.46\pm0.22$ & $98.20\pm0.09$ & $96.68\pm0.17$ & $79.53\pm0.37$ &  & $90.90\pm0.12$ & $97.27\pm0.12$ & $90.71\pm0.24$ &  \\
& 8 & $97.04\pm0.09$ & $91.07\pm0.21$ & $93.09\pm0.16$ & $98.54\pm0.05$ & $97.73\pm0.09$ & $80.88\pm0.25$ &  & $91.36\pm0.11$ & $97.85\pm0.08$ & $91.72\pm0.17$ &  \\
& 16 &$97.45\pm0.05$  &$91.59\pm0.17$  & $93.43\pm0.12$ & $98.67\pm0.03$ & $98.08\pm0.05$ & $81.63\pm0.17$ &  & $91.61\pm0.07$ & $98.12\pm0.04$ & $92.25\pm0.11$ &  \\

\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Result per dataset on one-class tasks. We compute the AUC score over 100 tasks and average the performance over 20 runs.}
\label{table:cross_domain_openset}
\end{table}

==> tables/cross_modal_openclass_with_deltas.tex <==
\newcommand{\uparrowgreen}{\tikz{\draw[green,->] (0,0) -- ++(0,0.3);}}
\newcommand{\downarrowred}{\tikz{\draw[red,->] (0,0.3) -- ++(0,-0.3);}}
\begin{table}[htbp]
\centering
 %\captionsetup{justification=centering}
\scalebox{0.484925}{\begin{tabular}{cc|c|ccccccccc|c}
\toprule
& \multirow{2}{*}{Method} & \multirow{2}{*}{Shots} & \multicolumn{10}{c}{Dataset}  \\ 
\cmidrule(r){4-13}
& & & Caltech~\cite{caltech101} & EuroSAT~\cite{eurosat} & Food~\cite{food101} & Flowers~\cite{oxford_flowers} & SUN397~\cite{sun397} & DTD~\cite{dtd} & Pets~\cite{oxford_pets} & Cars~\cite{stanford_cars} & UCF101~\cite{ucf101} & Average \\ 

\midrule
\multirow{5}{*}{\rotatebox{90}{AUROC}}&\multirow{5}{*}{\parbox{2cm}{\centering Baseline}} 
& 1 & $89.74\pm0.47$ & $81.34\pm0.66$ & $83.34\pm0.66$ & $90.92\pm0.42$ & $89.18\pm0.55$ & $71.23\pm0.66$ & $81.47\pm0.56$ & $90.31\pm0.42$ & $84.70\pm0.51$ & $84.70\pm0.54$ \\
&& 2 & $93.31\pm0.30$ &  $85.79\pm0.47$& $87.59\pm0.38$ & $94.66\pm0.21$ & $94.37\pm0.33$ & $76.36\pm0.56$ & $86.16\pm0.33$ & $94.28\pm0.29$ & $88.63\pm0.42$ & $89.02\pm0.36$\\
&& 4 & $94.95\pm0.19$ & $88.60\pm0.35$ & $89.54\pm0.27$ & $96.38\pm0.14$ & $96.47\pm0.18$ & $79.53\pm0.37$ &  $88.11\pm0.20$ & $96.04\pm0.17$ & $90.70\pm0.24$ & $91.15\pm0.23$ \\
&& 8 & $95.89\pm0.12$ & $89.85\pm0.23$ & $90.36\pm0.20$ & $97.09\pm0.09$ & $97.51\pm0.10$ & $80.88\pm0.25$ & $88.83\pm0.17$ & $96.78\pm0.11$ & $91.72\pm0.17$ &  $92.10\pm0.15$\\
&& 16 & $96.49\pm0.06$ & $90.39\pm0.17$ &$90.79\pm0.14$  & $97.51\pm0.04$ & $97.83\pm0.05$ & $81.63\pm0.17$ &  $89.21\pm0.11$ & $97.12\pm0.06$ & $92.25\pm0.11$ & $92.57\pm0.11$ \\
\midrule
\multirow{14}{*}{\rotatebox{90}{$\Delta\%$}}&\multirow{5}{*}{\parbox{2cm}{\centering Mean from text (M)}} 
& 1 & +$2.07\pm0.34$ & $0.00\pm0.00$ & +$0.68\pm0.56$ & +$0.48\pm0.36$ & +$2.83\pm0.36$ & +$0.17\pm0.63$ &  +$6.31\pm0.13$ & +$0.38\pm0.39$ & +$1.37\pm0.43$ & $1.59\pm0.36$\\ 
&& 2 & +$0.46\pm0.25$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$0.22\pm0.29$ & $0.00\pm0.00$ &  +$2.17\pm0.15$ & $0.00\pm0.00$ & +$0.11\pm0.40$ &  $0.33\pm0.12$\\ 
&& 4 & +$0.10\pm0.18$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ &  +$0.76\pm0.12$ & $0.00\pm0.00$ & $0.00\pm0.00$ &  $0.10\pm0.03$\\ 
&& 8 & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ &  +$0.37\pm0.11$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.04\pm0.01$ \\ 
&& 16 & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$0.18\pm0.08$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.02\pm0.01$ \\ 
\cmidrule(r){2-13}
& \multirow{5}{*}{\parbox{2cm}{\centering Covariance from text (C)}} 
& 1 & +$2.09\pm0.44$ & +$1.47\pm0.60$ & +$3.05\pm0.56$ & +$3.59\pm0.32$ & +$0.08\pm0.55$ & $0.00\pm0.00$ & +$4.57\pm0.43$ & +$1.97\pm0.33$ & $0.00\pm0.00$ &  +$1.86\pm0.36$\\ 
&& 2 & +$1.80\pm0.26$ & +$1.45\pm0.43$ & +$3.09\pm0.29$ & +$2.53\pm0.15$ & +$0.21\pm0.32$ & $0.00\pm0.00$ &  +$3.38\pm0.24$ & +$1.66\pm0.20$ & $0.00\pm0.00$ &  +$1.57\pm0.21$\\ 
&& 4 & +$\mathbf{1.49\pm0.15}$ & +$\mathbf{1.27\pm0.31}$ & +$\mathbf{2.92\pm0.22}$ & +$\mathbf{1.82\pm0.09}$ & +$\mathbf{0.21\pm0.17}$ & $\mathbf{0.00\pm0.00}$ &  +$\mathbf{2.76\pm0.14}$ & +$\mathbf{1.23\pm0.12}$ & $\mathbf{0.00\pm0.00}$ & +$\mathbf{1.30\pm0.13}$ \\ 
&& 8 & +$\mathbf{1.15\pm0.09}$ & +$\mathbf{1.22\pm0.21}$ & +$\mathbf{2.73\pm0.16}$ & +$\mathbf{1.45\pm0.05}$ & +$\mathbf{0.22\pm0.09}$ & $\mathbf{0.00\pm0.00}$ &  +$\mathbf{2.53\pm0.11}$ & +$\mathbf{1.07\pm0.08}$ & $\mathbf{0.00\pm0.00}$ & +$\mathbf{1.15\pm0.09}$ \\ 
&& 16 & +$\mathbf{0.96\pm0.05}$ & +$\mathbf{1.20\pm0.17}$ & +$\mathbf{2.64\pm0.12}$ & +$\mathbf{1.16\pm0.03}$ & +$\mathbf{0.25\pm0.05}$ & $\mathbf{0.00\pm0.00}$ & +$\mathbf{2.40\pm0.07}$ & +$\mathbf{1.00\pm0.04}$ & $\mathbf{0.00\pm0.00}$ & +$\mathbf{1.07\pm0.06}$\\  

\cmidrule(r){2-13}
&\multirow{5}{*}{\parbox{2cm}{\centering Mean and covariance from text (M\&C)}} 
& 1 & +$\mathbf{3.82\pm0.32}$ & +$\mathbf{1.47\pm0.60}$ & +$\mathbf{3.61\pm0.47}$ & +$\mathbf{3.99\pm0.27}$ & +$\mathbf{2.85\pm0.36}$ & +$\mathbf{0.17\pm0.63}$ &  +$\mathbf{8.43\pm0.12}$ & +$\mathbf{2.33\pm0.29}$ & +$\mathbf{1.37\pm0.43}$ & +$\mathbf{3.11\pm0.39}$ \\ 
&& 2 & +$\mathbf{2.07\pm0.21}$ & +$\mathbf{1.45\pm0.43}$ & +$\mathbf{3.09\pm0.29}$ & +$\mathbf{2.54\pm0.14}$ & +$\mathbf{0.34\pm0.30}$ & $0.00\pm0.00$ & +$\mathbf{4.18\pm0.12}$ & +$\mathbf{1.66\pm0.20}$ & +$\mathbf{0.11\pm0.40}$ & +$\mathbf{1.71\pm0.23}$ \\ 
&& 4 & +$\mathbf{1.52\pm0.14}$ & +$\mathbf{1.27\pm0.31}$ & +$\mathbf{2.92\pm0.22}$ & +$\mathbf{1.82\pm0.09}$ & +$\mathbf{0.21\pm0.17}$ & $0.00\pm0.00$ &  +$\mathbf{2.79\pm0.12}$ & +$\mathbf{1.23\pm0.12}$ & +$0.01\pm0.00$ & +$\mathbf{1.31\pm0.13}$ \\ 
&& 8 & +$\mathbf{1.15\pm0.09}$ & +$\mathbf{1.22\pm0.21}$ & +$\mathbf{2.73\pm0.16}$ & +$\mathbf{1.45\pm0.05}$ & +$\mathbf{0.22\pm0.09}$ & $0.00\pm0.00$ &  +$\mathbf{2.53\pm0.11}$ & +$\mathbf{1.07\pm0.08}$ & $0.00\pm0.00$ & +$\mathbf{1.15\pm0.09}$ \\ 
&& 16 & +$\mathbf{0.96\pm0.05}$ & +$\mathbf{1.20\pm0.17}$ & +$\mathbf{2.64\pm0.12}$ & +$\mathbf{1.16\pm0.03}$ & +$\mathbf{0.25\pm0.05}$ & $0.00\pm0.00$ & +$\mathbf{2.40\pm0.07}$ & +$\mathbf{1.00\pm0.04}$ & $0.00\pm0.00$ & +$\mathbf{1.07\pm0.06}$ \\ 

\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Results per dataset on one-class tasks. We compute the AUROC score over 100 tasks and average the performance over 20 runs. We report the score difference with respect to the Baseline for different number of shots. We highlight the best performance gains compared to the baseline.}
\label{table:cross_domain_openset_with_deltas}
\end{table}

==> tables/cross_modal_openset_withdeltas_old.tex <==
\newcommand{\uparrowgreen}{\tikz{\draw[green,->] (0,0) -- ++(0,0.3);}}
\newcommand{\downarrowred}{\tikz{\draw[red,->] (0,0.3) -- ++(0,-0.3);}}
\begin{table}[htbp]
\centering
 %\captionsetup{justification=centering}
\scalebox{0.4725}{\begin{tabular}{cc|c|cccccccccc|c}
\toprule
& \multirow{2}{*}{Method} & \multirow{2}{*}{Shots} & \multicolumn{11}{c}{Dataset}  \\ 
\cmidrule(r){4-14}
& & & Caltech~\cite{caltech101} & EuroSAT~\cite{eurosat} & Food~\cite{food101} & Flowers~\cite{oxford_flowers} & SUN397~\cite{sun397} & DTD~\cite{dtd} & Aircraft~\cite{aircraft} & Pets~\cite{oxford_pets} & Cars~\cite{stanford_cars} & UCF101~\cite{ucf101} & Average \\ 

\midrule
\multirow{5}{*}{\rotatebox{90}{Accuracy}}&\multirow{5}{*}{\parbox{2cm}{\centering Baseline}} 
& 1 & $89.74\pm0.47$ & $81.34\pm0.66$ & $83.34\pm0.66$ & $90.92\pm0.42$ & $89.18\pm0.55$ & $71.23\pm0.66$ & $72.04\pm0.63$ & $81.47\pm0.56$ & $90.31\pm0.42$ & $84.70\pm0.51$ & $83.43\pm0.55$ \\
&& 2 & $93.31\pm0.30$ &  $85.79\pm0.47$& $87.59\pm0.38$ & $94.66\pm0.21$ & $94.37\pm0.33$ & $76.36\pm0.56$ & $76.41\pm0.45$ & $86.16\pm0.33$ & $94.28\pm0.29$ & $88.63\pm0.42$ & $87.76\pm0.37$ \\
&& 4 & $94.95\pm0.19$ & $88.60\pm0.35$ & $89.54\pm0.27$ & $96.38\pm0.14$ & $96.47\pm0.18$ & $79.53\pm0.37$ & $78.65\pm0.32$ & $88.11\pm0.20$ & $96.04\pm0.17$ & $90.70\pm0.24$ & $89.90\pm0.24$ \\
&& 8 & $95.89\pm0.12$ & $89.85\pm0.23$ & $90.36\pm0.20$ & $97.09\pm0.09$ & $97.51\pm0.10$ & $80.88\pm0.25$ & $79.58\pm0.21$ & $88.83\pm0.17$ & $96.78\pm0.11$ & $91.72\pm0.17$ &  $90.85\pm0.16$\\
&& 16 & $96.49\pm0.06$ & $90.39\pm0.17$ &$90.79\pm0.14$  & $97.51\pm0.04$ & $97.83\pm0.05$ & $81.63\pm0.17$ & $80.03\pm0.14$ & $89.21\pm0.11$ & $97.12\pm0.06$ & $92.25\pm0.11$ & $91.32\pm0.11$ \\
\midrule
\multirow{14}{*}{\rotatebox{90}{$\Delta\%$}}&\multirow{5}{*}{\parbox{2cm}{\centering Mean from text (M)}} 
& 1 & +$2.07\pm0.34$ & $0.00\pm0.00$ & +$0.68\pm0.56$ & +$0.48\pm0.36$ & +$2.83\pm0.36$ & +$0.17\pm0.63$ & $0.00\pm0.00$ & +$6.31\pm0.13$ & +$0.38\pm0.39$ & +$1.37\pm0.43$ & $1.43\pm0.32$ \\ 
&& 2 & +$0.46\pm0.25$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$0.22\pm0.29$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$2.17\pm0.15$ & $0.00\pm0.00$ & +$0.11\pm0.40$ &  $0.30\pm0.11$\\ 
&& 4 & +$0.10\pm0.18$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$0.76\pm0.12$ & $0.00\pm0.00$ & $0.00\pm0.00$ &  $0.09\pm0.03$\\ 
&& 8 & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$0.37\pm0.11$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.04\pm0.01$ \\ 
&& 16 & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.00\pm0.00$ & +$0.18\pm0.08$ & $0.00\pm0.00$ & $0.00\pm0.00$ & $0.02\pm0.01$ \\ 
\cmidrule(r){2-14}
& \multirow{5}{*}{\parbox{2cm}{\centering Covariance from text (C)}} 
& 1 & +$2.09\pm0.44$ & +$1.47\pm0.60$ & +$3.05\pm0.56$ & +$3.59\pm0.32$ & +$0.08\pm0.55$ & $0.00\pm0.00$ & +$1.02\pm0.69$ & +$4.57\pm0.43$ & +$1.97\pm0.33$ & $0.00\pm0.00$ &  +$1.78\pm0.39$\\ 
&& 2 & +$1.80\pm0.26$ & +$1.45\pm0.43$ & +$3.09\pm0.29$ & +$2.53\pm0.15$ & +$0.21\pm0.32$ & $0.00\pm0.00$ & +$0.89\pm0.45$ & +$3.38\pm0.24$ & +$1.66\pm0.20$ & $0.00\pm0.00$ &  +$1.50\pm0.23$\\ 
&& 4 & +$1.49\pm0.15$ & +$1.27\pm0.31$ & +$2.92\pm0.22$ & +$1.82\pm0.09$ & +$0.21\pm0.17$ & $0.00\pm0.00$ & +$0.81\pm0.31$ & +$2.76\pm0.14$ & +$1.23\pm0.12$ & +$0.01\pm0.00$ & +$1.25\pm0.15$ \\ 
&& 8 & +$1.15\pm0.09$ & +$1.22\pm0.21$ & +$2.73\pm0.16$ & +$1.45\pm0.05$ & +$0.22\pm0.09$ & $0.00\pm0.00$ & +$0.85\pm0.21$ & +$2.53\pm0.11$ & +$1.07\pm0.08$ & $0.00\pm0.00$ & +$\mathbf{1.12\pm0.10}$ \\ 
&& 16 & +$0.96\pm0.05$ & +$1.20\pm0.17$ & +$2.64\pm0.12$ & +$1.16\pm0.03$ & +$0.25\pm0.05$ & $0.00\pm0.00$ & +$0.89\pm0.14$ & +$2.40\pm0.07$ & +$1.00\pm0.04$ & $0.00\pm0.00$ & +$\mathbf{1.05\pm0.07}$\\  

\cmidrule(r){2-14}
&\multirow{5}{*}{\parbox{2cm}{\centering Mean and covariance from text (M\&C)}} 
& 1 & +$3.82\pm0.32$ & +$1.47\pm0.60$ & +$3.61\pm0.47$ & +$3.99\pm0.27$ & +$2.85\pm0.36$ & +$0.17\pm0.63$ & +$1.17\pm0.63$ & +$8.43\pm0.12$ & +$2.33\pm0.29$ & +$1.37\pm0.43$ & +$\mathbf{2.92\pm0.41}$ \\ 
&& 2 & +$2.07\pm0.21$ & +$1.45\pm0.43$ & +$3.09\pm0.29$ & +$2.54\pm0.14$ & +$0.34\pm0.30$ & $0.00\pm0.00$ & +$0.89\pm0.45$ & +$4.18\pm0.12$ & +$1.66\pm0.20$ & +$0.11\pm0.40$ & +$\mathbf{1.63\pm0.25}$ \\ 
&& 4 & +$1.52\pm0.14$ & +$1.27\pm0.31$ & +$2.92\pm0.22$ & +$1.82\pm0.09$ & +$0.21\pm0.17$ & $0.00\pm0.00$ & +$0.81\pm0.31$ & +$2.79\pm0.12$ & +$1.23\pm0.12$ & +$0.01\pm0.00$ & +$\mathbf{1.26\pm0.15}$ \\ 
&& 8 & +$1.15\pm0.09$ & +$1.22\pm0.21$ & +$2.73\pm0.16$ & +$1.45\pm0.05$ & +$0.22\pm0.09$ & $0.00\pm0.00$ & +$0.85\pm0.21$ & +$2.53\pm0.11$ & +$1.07\pm0.08$ & $0.00\pm0.00$ & +$\mathbf{1.12\pm0.10}$ \\ 
&& 16 & +$0.96\pm0.05$ & +$1.20\pm0.17$ & +$2.64\pm0.12$ & +$1.16\pm0.03$ & +$0.25\pm0.05$ & $0.00\pm0.00$ & +$0.89\pm0.14$ & +$2.40\pm0.07$ & +$1.00\pm0.04$ & $0.00\pm0.00$ & +$\mathbf{1.05\pm0.07}$ \\ 

\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Result per dataset on one-class tasks. We compute the AUC score over 100 tasks and average the performance over 20 runs. We report the score difference with respect to the Baseline for different number of shots.}
\label{table:cross_domain_openset_with_deltas}
\end{table}

==> tables/cross_modal_table.tex <==
\newcommand{\uparrowgreen}{\tikz{\draw[green,->] (0,0) -- ++(0,0.3);}}
\newcommand{\downarrowred}{\tikz{\draw[red,->] (0,0.3) -- ++(0,-0.3);}}
\begin{table}[htbp]
\label{table:MSE}
\centering
 %\captionsetup{justification=centering}
\scalebox{0.73}{\begin{tabular}{c|c|cccccccccc|c}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Shots} & \multicolumn{11}{c}{Dataset}  \\ 
\cmidrule(r){3-13}
& & Caltech & EuroSAT & Food & Flowers & SUN397 & DTD  & Aircraft & Pets & Cars & UCF101 & Average \\ 
\midrule
\parbox{2cm}{\centering Zero-Shot CLIP} &  &  &  &  &  &  &  &  &  &  &  
& \\ 
\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Cross-Modal Linear Probe}} 
& 1 & 88.627 & 59.605 & 76.19 & 80.823 & 62.121 &  &  &  &  &  &  \\
& 2 & 88.695 & 67.58 & 77.274 & 86.006 & 64.856 &  &  &  &  &  &  \\
& 4 & 91.007 & 73.247 & 77.612 & 90.432 & 66.945 &  &  &  &  &  &  \\
& 8 & 92.211 & 80.049 & 77.853 & 93.815 & 69.011 &  &  &  &  &  &  \\
& 16 & 93.009 & 83.704 & 78.504 & 96.211 & 70.7 &  &  &  &  &  &  \\
\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Cross-Modal Linear Probe + Predicted Covariance}} 
& 1 & 88.993 \uparrowgreen & 59.897 \uparrowgreen & 77.406 \uparrowgreen & 81.391 \uparrowgreen & 62.427 \uparrowgreen &  &  &  &  &  &  \\
& 2 & 89.52 \uparrowgreen & 68.169 \uparrowgreen & 77.388 \uparrowgreen & 86.358 \uparrowgreen & 64.996 \uparrowgreen &  &  &  &  &  &  \\
& 4 & 91.373 \uparrowgreen & 74.807 \uparrowgreen & 77.67 \uparrowgreen & 90.946 \uparrowgreen & 67.207 \uparrowgreen &  &  &  &  &  &  \\
& 8 & 92.373 & 80.564 & 78.417 & 94.072 & 69.157 &  &  &  &  &  &  \\
& 16 & 92.874 & 85.251 & 78.677 & 96.292 & 70.86 &  &  &  &  &  &  \\
 \midrule
\multirow{5}{*}{\parbox{2cm}{\centering Cross-Modal Linear Probe + Oracle Covariance}} 
& 1 & 89.479 & 60.21 & 77.455 &  & 62.532 &  &  &  &  &  &  \\
& 2 & 89.642 & 68.407 & 77.466 &  & 65.056 &  &  &  &  &  &  \\
& 4 & 91.494 & 75.177 & 78.112 &  & 67.211 &  &  &  &  &  &  \\
& 8 & 92.549 & 81.008 & 78.491 &  & 69.214 &  &  &  &  &  &  \\
& 16 & 93.617 & 85.436 & 78.932 &  & 71.071 &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Results per dataset.}
\end{table}

==> tables/cross_modal_table_multi_class_with_deltas.tex <==
\newcommand{\uparrowgreen}{\tikz{\draw[green,->] (0,0) -- ++(0,0.3);}}
\newcommand{\downarrowred}{\tikz{\draw[red,->] (0,0.3) -- ++(0,-0.3);}}
\begin{table}[htbp]
\label{table:MSE}
\centering
 %\captionsetup{justification=centering}
\scalebox{0.4525}{\begin{tabular}{cc|c|ccccccccc|c}
\toprule
& \multirow{2}{*}{Method} & \multirow{2}{*}{Shots} & \multicolumn{10}{c}{Dataset}  \\ 
\cmidrule(r){4-13}
& & & Caltech~\cite{caltech101} & EuroSAT~\cite{eurosat} & Food~\cite{food101} & Flowers~\cite{oxford_flowers} & SUN397~\cite{sun397} & DTD~\cite{dtd} & Pets~\cite{oxford_pets} & Cars~\cite{stanford_cars} & UCF101~\cite{ucf101} & Average \\ 
\cmidrule(r){1-13}
\multicolumn{2}{c}{\parbox{3cm}{\centering Zero-Shot CLIP}} & 0 & 82.39 & 36.01 & 75.72 & 62.28 & 56.60 & 40.01 &  79.59 & 51.91 & 59.42 & 60.43\\ 
\midrule

\multirow{5}{*}{\rotatebox{90}{Accuracy}} & \multirow{5}{*}{\parbox{2cm}{\centering Baseline}} 
& 1 & $62.07\pm0.19$ & $47.80\pm0.34$ & $27.55\pm0.09$ & $52.25\pm0.13$ & $28.15\pm0.05$ & $26.11\pm0.15$ & $26.69\pm0.15$ & $21.62\pm0.06$ & $36.89\pm0.12$ &$36.57\pm0.14$\\
& & 2 & $74.95\pm0.09$ & $58.30\pm0.27$ &$40.33\pm0.08$ &$69.10\pm0.10$ & $41.42\pm0.04$ & $37.64\pm0.13$  & $38.28\pm0.14$ & $33.18\pm0.06$ & $50.08\pm0.09$ &$49.25\pm0.11$\\
& & 4 & $81.31\pm0.06$ & $66.07\pm0.17$ & $51.67\pm0.06$ & $80.49\pm0.06$ & $51.89\pm0.03$ & $47.49\pm0.10$  & $49.65\pm0.13$ & $44.02\pm0.05$ & $58.80\pm0.08$ &$59.04\pm0.08$\\
& & 8 & $84.61\pm0.04$ & $70.67\pm0.12$ & $59.72\pm0.04$ & $86.52\pm0.04$ & $58.59\pm0.02$ & $54.17\pm0.07$  & $58.63\pm0.10$ & $52.53\pm0.04$ & $64.23\pm0.06$ &$65.52\pm0.06$\\
& & 16 & $86.34\pm0.08$ & $73.49\pm0.09$ & $64.68\pm0.03$ & $89.59\pm0.03$ & $62.46\pm0.01$ & $58.21\pm0.05$ & $65.23\pm0.28$ & $65.18\pm0.09$ & $67.48\pm0.05$ &$70.68\pm0.05$\\

\cmidrule(r){1-13}
\multirow{14}{*}{\rotatebox{90}{$\Delta\%$}}  & \multirow{5}{*}{\parbox{2cm}{\centering Mean  from text}} 
& 1 & +$16.46\pm0.08$ & +$0.82\pm0.39$ & +$13.80\pm0.12$ & +$6.58\pm0.14$ & +$17.22\pm0.05$ & +$6.94\pm0.18$  & +$26.56\pm0.24$ & +$5.26\pm0.08$ & +$9.98\pm0.12$ & +$11.51\pm0.16$ \\
&& 2 & +$6.30\pm0.06$ & +$0.33\pm0.28$ & +$8.09\pm0.09$ & +$2.58\pm0.09$ & +$9.00\pm0.04$ & +$3.62\pm0.13$  & +$19.74\pm0.17$ & +$2.04\pm0.06$ & +$4.06\pm0.09$ & +$06.20\pm0.11$ \\
&& 4 & +$2.32\pm0.05$ & -$0.07\pm0.20$ & +$3.85\pm0.06$ & +$0.75\pm0.06$ & +$3.66\pm0.03$ & +$1.49\pm0.10$ & +$13.40\pm0.14$ & +$0.58\pm0.05$ & +$1.53\pm0.07$ & +$03.06\pm0.08$ \\
&& 8 & +$0.76\pm0.04$ & -$0.19\pm0.14$ & +$1.57\pm0.05$ & +$0.20\pm0.05$ & +$1.30\pm0.02$ & +$0.55\pm0.07$ & +$8.91\pm0.14$ & +$0.13\pm0.04$ & +$0.51\pm0.06$ & +$01.53\pm0.07$ \\
&& 16 & +$0.21\pm0.09$ & -$0.33\pm0.11$ & +$0.67\pm0.04$ & +$0.04\pm0.03$ & +$0.43\pm0.02$ & +$0.28\pm0.06$ & +$5.61\pm0.44$ & +$5.76\pm0.13$ & +$0.15\pm0.05$ & +$0.91\pm0.06$ \\
\cmidrule(r){2-13}
&\multirow{5}{*}{\parbox{2cm}{\centering Covariance from text}} 
& 1 & +$1.56\pm0.21$ & +$0.84\pm0.35$ & +$4.06\pm0.13$ & +$6.34\pm0.15$ & +$0.74\pm0.05$ & +$1.79\pm0.17$  & +$6.64\pm0.25$ & +$4.93\pm0.09$ & +$1.48\pm0.14$ & +$03.15\pm0.17$ \\
&& 2 & +$2.92\pm0.10$ & +$1.52\pm0.28$ & +$6.72\pm0.10$ & +$6.84\pm0.10$ & +$2.16\pm0.05$ & +$3.75\pm0.15$  & +$11.10\pm0.20$ & +$7.58\pm0.07$ & +$3.50\pm0.10$ & +$05.12\pm0.13$ \\
&& 4 & +$2.85\pm0.06$ & +$1.97\pm0.18$ & +$7.41\pm0.06$ & +$5.35\pm0.06$ & +$3.21\pm0.03$ & +$5.27\pm0.11$  & +$13.29\pm0.15$ & +$8.72\pm0.05$ & +$4.55\pm0.08$ & +$05.85\pm0.09$ \\
&& 8 & +$2.44\pm0.04$ & +$2.03\pm0.14$ & +$6.71\pm0.04$ & +$3.88\pm0.05$ & +$3.59\pm0.02$ & +$5.44\pm0.08$  & +$12.60\pm0.14$ & +$8.77\pm0.04$ & +$4.98\pm0.06$ & +$05.60\pm0.07$ \\
&& 16 & +$2.29\pm0.09$ & +$1.99\pm0.12$ & +$5.80\pm0.04$ & +$2.95\pm0.04$ & +$3.59\pm0.02$ & +$5.33\pm0.07$ & +$11.31\pm0.36$ & +$11.22\pm0.12$  & +$5.11\pm0.05$ & +$04.82\pm0.07$ \\ 
\cmidrule(r){2-13}
&\multirow{5}{*}{\parbox{2cm}{\centering Mean and covariance from text}} 
& 1 & +$\mathbf{21.03\pm0.08}$ & +$\mathbf{2.20\pm0.38}$ & +$\mathbf{25.57\pm0.12}$ & +$\mathbf{14.90\pm0.14}$ & +$\mathbf{22.14\pm0.05}$ & +$\mathbf{14.05\pm0.20}$  & +$\mathbf{37.86\pm0.28}$ & +$\mathbf{16.14\pm0.09}$ & +$\mathbf{14.94\pm0.12}$ & +$\mathbf{18.76\pm0.16}$ \\
&& 2 & +$\mathbf{10.27\pm0.05}$ & +$\mathbf{2.04\pm0.30}$ & +$\mathbf{18.42\pm0.08}$ & +$\mathbf{9.82\pm0.09}$ & +$\mathbf{13.74\pm0.04}$ & +$\mathbf{10.45\pm0.15}$  & +$\mathbf{31.86\pm0.19}$ & +$\mathbf{11.22\pm0.07}$ & +$\mathbf{9.48\pm0.10}$ & +$\mathbf{13.03\pm0.12}$ \\
&& 4 & +$\mathbf{5.76\pm0.04}$ & +$\mathbf{2.21\pm0.21}$ & +$\mathbf{12.49\pm0.06}$ & +$\mathbf{6.21\pm0.06}$ & +$\mathbf{8.23\pm0.03}$ & +$\mathbf{8.15\pm0.11}$  & +$\mathbf{25.80\pm0.13}$ & +$\mathbf{9.67\pm0.05}$ & +$\mathbf{7.27\pm0.08}$ & +$\mathbf{09.53\pm0.09}$ \\
&& 8 & +$\mathbf{3.71\pm0.04}$ & +$\mathbf{2.09\pm0.16}$ & +$\mathbf{8.78\pm0.05}$ & +$\mathbf{4.21\pm0.04}$ & +$\mathbf{5.56\pm0.03}$ & +$\mathbf{6.71\pm0.08}$ & +$\mathbf{20.42\pm0.12}$ & +$\mathbf{9.06\pm0.04}$ & +$\mathbf{6.29\pm0.06}$ & +$\mathbf{07.43\pm0.07}$ \\
&& 16 & +$\mathbf{2.81\pm0.11}$ & +$\mathbf{2.02\pm0.14}$ & +$\mathbf{6.74\pm0.04}$ & +$\mathbf{3.13\pm0.04}$ & +$\mathbf{4.46\pm0.02}$ & +$\mathbf{6.10\pm0.06}$ & +$\mathbf{16.30\pm0.37}$ & +$\mathbf{15.99\pm0.12}$ & +$\mathbf{5.91\pm0.05}$ & +$\mathbf{5.94\pm0.07}$ \\ 
\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Results per dataset. We report the performance across $10^2$ tasks of Zero-shot CLIP and the baseline, for other methods we report the average difference to the baseline. We observe that combining and mean and covariance (M\&C) consistently improves the baseline.}
\label{table:cross_domain_multiclass_with_deltas}
\end{table}


==> tables/cross_modal_table_multiclass.tex <==
\newcommand{\uparrowgreen}{\tikz{\draw[green,->] (0,0) -- ++(0,0.3);}}
\newcommand{\downarrowred}{\tikz{\draw[red,->] (0,0.3) -- ++(0,-0.3);}}
\begin{table}[htbp]
\label{table:MSE}
\centering
 %\captionsetup{justification=centering}
\scalebox{0.52}{\begin{tabular}{c|c|cccccccccc|c}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Shots} & \multicolumn{11}{c}{Dataset}  \\ 
\cmidrule(r){3-13}
& & Caltech & EuroSAT & Food & Flowers & SUN397 & DTD  & Aircraft & Pets & Cars & UCF101 & Average \\ 
\midrule
\parbox{2cm}{\centering Zero-Shot CLIP} & 0 & 82.39 & 36.01 & 75.72 & 62.28 & 56.60 & 40.01 &  & 79.59 & 51.91 & 59.42 & \\ 
\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Baseline}} 
& 1 & $62.07\pm0.19$ & $47.80\pm0.34$ & $27.55\pm0.09$ & $52.25\pm0.13$ & $28.15\pm0.05$ & $26.11\pm0.15$ &  & $26.69\pm0.15$ & $21.62\pm0.06$ & $36.89\pm0.12$ &  \\
& 2 & $74.95\pm0.09$ & $58.30\pm0.27$ &$40.33\pm0.08$ &$69.10\pm0.10$ & $41.42\pm0.04$ & $37.64\pm0.13$ &  & $38.28\pm0.14$ & $33.18\pm0.06$ & $50.08\pm0.09$ &  \\
& 4 & $81.31\pm0.06$ & $66.07\pm0.17$ & $51.67\pm0.06$ & $80.49\pm0.06$ & $51.89\pm0.03$ & $47.49\pm0.10$ &  & $49.65\pm0.13$ & $44.02\pm0.05$ & $58.80\pm0.08$ &  \\
& 8 & $84.61\pm0.04$ & $70.67\pm0.12$ & $59.72\pm0.04$ & $86.52\pm0.04$ & $58.59\pm0.02$ & $54.17\pm0.07$ &  & $58.63\pm0.10$ & $52.53\pm0.04$ & $64.23\pm0.06$ &  \\
& 16 & & $73.49\pm0.09$ & $64.68\pm0.03$ & $89.59\pm0.03$ & $62.46\pm0.01$ & $58.21\pm0.05$ &  & $65.18\pm0.09$ &  & $67.48\pm0.05$ &  \\
\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Mean  from text}} 
& 1 &  &  &  &  &  &  &  &  &  &  &  \\
& 2 &  & &  &  &  &  &  &  &  &  &  \\
& 4 &  &  &  &  &  &  &  &  &  &  &  \\
& 8 &  &  &  &  &  &  &  &  &  &  &  \\
& 16 &  &  &  &  &  &  &  &  &  &  &  \\
 \midrule
\multirow{5}{*}{\parbox{2cm}{\centering Covariance from text}} 
& 1 &  &  &  &  &  &  &  &  &  &  &  \\
& 2 &  & &  &  &  &  &  &  &  &  &  \\
& 4 &  &  &  &  &  &  &  &  &  &  &  \\
& 8 &  &  &  &  &  &  &  &  &  &  &  \\
& 16 &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow{5}{*}{\parbox{2cm}{\centering Mean and covariance from text}} 
& 1 & $83.10\pm0.08$& $50.00\pm0.38$ & $53.12\pm0.12$ & $67.15\pm0.14$ & $50.29\pm0.05$ & $40.16\pm0.20$ &  & $64.55\pm0.28$ & $37.76\pm0.09$ & $51.83\pm0.12$ &  \\
& 2 & $85.22\pm0.05$& $60.34\pm0.30$ &$58.75\pm0.08$ & $78.92\pm0.09$ & $55.16\pm0.04$ & $48.09\pm0.15$ &  & $70.14\pm0.19$ & $44.40\pm0.07$ & $59.56\pm0.10$ &  \\
& 4 & $87.07\pm0.04$ &  $68.28\pm0.21$& $64.16\pm0.06$ & $86.70\pm0.06$ & $60.12\pm0.03$ & $55.64\pm0.11$ &  & $75.45\pm0.13$ & $53.69\pm0.05$ & $66.07\pm0.08$ &  \\
& 8 & $88.32\pm0.04$ & $72.76\pm0.16$ & $68.50\pm0.05$ & $90.73\pm0.04$ & $64.15\pm0.03$ & $60.88\pm0.08$ &  & $79.05\pm0.12$ & $61.59\pm0.04$ & $70.52\pm0.06$ &  \\
& 16 &  & $75.51\pm0.14$ & $71.42\pm0.04$ & $92.72\pm0.04$ & $66.92\pm0.02$ & $64.31\pm0.06$ &  & $81.17\pm0.12$ &  & $73.39\pm0.05$ &  \\
\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Results per dataset.}
\end{table}


%& 1 & $64.95\pm0.97$ &  $45.39\pm4.15$ & $31.90\pm1.01$ & $58.44\pm1.25$ & $28.83\pm0.41$ & $27.88\pm1.59$ &  & $33.51\pm2.48$ & $26.88\pm0.77$ & $38.03\pm1.25$ &  \\
%& 2 & $77.09\pm0.82$ & $61.04\pm2.14$ & $47.03\pm0.73$ & $76.12\pm0.96$ & $43.07\pm0.49$ & $41.49\pm1.90$ &  & $49.47\pm1.71$ & $40.12\pm1.11$ & $53.98\pm1.23$ &  \\
%& 4 & $83.89\pm0.55$ &  $67.37\pm1.88$ & $59.11\pm0.45$ & $85.89\pm0.52$ & $55.28\pm0.32$ & $52.70\pm1.18$ &  & $63.11\pm1.69$ & $52.98\pm0.47$ & $62.68\pm0.69$ &  \\
%& 8 & $86.99\pm0.60$ &  $72.83\pm1.28$ & $66.32\pm0.38$ & $90.66\pm0.49$ & $62.29\pm0.26$ & $59.68\pm1.36$ &  & $71.13\pm1.22$ & $61.46\pm0.34$ & $69.20\pm0.63$ &  \\
%& 16 &  &  $75.19\pm0.96$ & $70.67\pm0.23$ & $92.76\pm0.32$ & $66.00\pm0.12$ & $63.36\pm0.48$ &  & $76.20\pm1.51$ &  & $72.49\pm0.64$ &  \\

==> tables/cross_modal_table_pivot.tex <==
\begin{table}[htbp]
\label{table:MSE}
\centering
\scalebox{0.8}{
\begin{tabular}{c|c|p{2cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Shots} & \multirow{2}{1.5cm}{\centering \parbox{2cm}{\centering Zero-Shot CLIP}} & \multicolumn{3}{c}{Cross-Modal Linear Probe} \\
\cmidrule(r){4-6}
 &  &  & \parbox{2.5cm}{\centering Basic} & \parbox{2.5cm}{\centering + Predicted Covariance} & \parbox{3cm}{\centering + GT Covariance} \\
\midrule
\multirow{6}{*}{Caltech}
 & 0 & 1 & - & - & - \\
 & 1 & - & 0 & 0 & 0 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
\midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
\midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
 \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
 \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
 \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
 \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
  \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
  \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
  \midrule
\multirow{6}{*}{DTD}
 & 0 & 1 & - & - & - \\
 & 1 & - & 1 & 1 & 1 \\
 & 2 & - & 1 & 1 & 1 \\
 & 4 & - & 1 & 1 & 1 \\
 & 8 & - & 1 & 1 & 1 \\
 & 16 & - & 1 & 1 & 1 \\
% Continue for each dataset
\bottomrule
\end{tabular}}
\vspace{2mm}

\caption{Mean Squared Error of predictions from ImageNet-1k and iNaturalist, pivoted}
\end{table}

